Lagrangian antisurgery

We describe an operation which modifies a Lagrangian submanifold $L$ in a symplectic manifold $(M, \omega)$ such as to produce a new immersed Lagrangian submanifold $L'$, which as a smooth manifold is obtained by surgery along a framed sphere in $L$. Intuitively, this can be described as collapsing an isotropic disc with boundary on $L$ to a point. The inverse operation generalizes classical Lagrangian surgery. We also describe corresponding immersed Lagrangian cobordisms between $L$ and $L'$ . After removal of their singular locus, we obtain examples of embedded Lagrangian cobordisms with precisely two ends. As an application, we use this construction to produce interesting examples of Lagrangian cobordisms between Clifford and Chekanov tori.

==> 6-Examples.tex <==
\section{Other examples}
\label{sec:examples}

\subsection{The case $k = 0$}
Lagrangian 0-antisurgery can be performed on any Lagrangian $L$ in any
symplectic manifold $M$, since isotropic surgery discs of dimension
one are always for free: They are simply embedded paths $\gamma: D^1
\to M$ hitting $L$ cleanly at their ends and nowhere else. We give two
simple applications in the lowest dimensions $n = 1,2$ (for $n = 1$,
this case coincides of course with the previously discussed case $k =
n-1$).

\subsubsection{Curves}
\label{sec:0-antisurgery-curves} Consider a simple closed curve
$\alpha$ on a surface $\Sigma$ and a surgery disc $\gamma: D^1 \to
\Sigma$ for $\alpha$. Let $\beta$ be a simple closed curve which is
obtained from $\gamma$ by connecting $\gamma(0)$ and $\gamma(1)$ by a
segment on $\alpha$. The geometric intersection number
$i(\alpha,\beta)$ can either be 0 or 1, depending on whether $\gamma$
approaches $\alpha$ from the same or two different sides at its
ends. If $i(\alpha,\beta) = 0$, the result of first antisurgering
$\alpha$ along $\gamma$ and then resolving the double point is a curve
$\widetilde \alpha$ isotopic but generally not Hamiltonian isotopic to
$\alpha$ (for one of the two possible resolutions; the other one leads
to a non-connected result). If $i(\alpha,\beta) = 1$, the result is
the squared Dehn twist of $\alpha$ about a curve $\widetilde \beta$
isotopic to $\beta$. The corresponding Lagrangian cobordisms
\begin{equation*}
    \widetilde \alpha \leadsto \alpha \quad \text{resp.} \quad
    \tau_{\widetilde \beta}^2(\alpha) \leadsto \alpha
\end{equation*}
are non-orientable in both cases.

\subsubsection{Surfaces}
Lagrangian 0-antisurgery applied to a Lagrangian surface $L$ in a
symplectic 4-manifold $M$ yields a Lagrangian immersion of a surface
$L'$ with $\chi(L') = \chi(L) - 2$. For example, if we start with a
torus in $\mathbb R^4$, iterating this procedure $g-1$ times produces
of a genus $g$ surface with exactly $g-1$ double points. By resolving
these double points, we get Lagrangian embeddings into $\mathbb R^4$
of all non-orientable surfaces whose Euler characteristic is divisible
by $4$, and corresponding non-orientable cobordisms. The existence of
such embeddings and immersions was of course known before, see e.g.\
\cite{Audin-Lalonde-Polterovich}.

\subsection{Middle-dimensional cases}
\label{sec:middle-dimens-cases}

\subsubsection{Monotone examples in $\mathbb CP^n$}
\label{sec:examples-cpn}
[\textbf{TODO} Not possible to make anything monotone, but maybe this
way of constructing examples is still somehow worth mentioning.]

We will view $\mathbb CP^n$ as a compactification of $D^*\mathbb
RP^n$, the unit cotangent bundle of $\mathbb RP^n$ with respect to the
round metric, which is obtained by collapsing the cogeodesic orbits on
the unit cosphere bundle to points (i.e., by a symplectic cut in the
sense of \cite{Lerman--Symplectic-cuts}).
For $r \in (0,1)$, let $S_r \subset D_p^*\mathbb RP^n$ be the sphere
of radius $r$ in the codisc fibre over $p = [0:\dots:0:1] \in \mathbb
RP^n$. Flowing $S_r$ around by the cogeodesic flow yields a Lagrangian
\begin{equation*}
    L_r \cong S^1 \times S^{n-1}
\end{equation*}
which as a Lagrangian submanifold of $\mathbb CP^n$ is monotone if and
only if $r = \frac{n-1}{n+1}$ (see the proof of Theorem
\ref{thm:monotone-examples-CPn} below).
By construction, the sphere $S_r \subset L_r$ bounds a Lagrangian disc
$D_r$. If we perform $k$-antisurgery along some $(k+1)$-dimensional
subdisc of $D_r$ and then remove the double point thus created, we
obtain an embedded Lagrangian $L_r^\natural \subset \mathbb CP^n$
which is diffeomorphic to
\begin{equation*}
    (S^{k+1} \times S^{n-k-1}) \# 2 P^n \quad \text{resp.}\quad
    (S^{k+1} \times S^{n-k-1}) \# P^n \#Q^n
\end{equation*}
(depending on $n$ and $k$, see Section \ref{sec:orientability}), and
an embedded Lagrangian cobordism $V^\natural: L_r^\natural \leadsto
L_r$. [\textbf{TODO} Only get a cobordism for one of them.]

\begin{rmk}
    The Lagrangian $L_r \cong S^1 \times S^{n-1}$ can also be viewed as
    the Lagrangian circle bundle over the trace of the polarization of
    $\mathbb CP^n$ given by the quadric $\Sigma = \{z_1^2 + \dots +
    z_{n+1}^2 = 0\}$, in the sense of \cite{Biran--Lagr-barriers,
        Biran_LagrangianNonIntersections2006}. This construction also
    yields examples of Lagrangians with Lagrangian surgery discs in
    other polarized K\"ahler manifolds.
\end{rmk}

\subsubsection{Lagrangian circle bundles}
\label{sec:polar-kahl-manif} 
Biran's construction of Lagrangian circle bundles in polarized
K\"ahler manifolds \cite{Biran--Lagr-barriers,
    Biran_LagrangianNonIntersections2006} yield examples for
Lagrangians containing spheres with associated Lagrangian surgery
discs.

By a polarized K\"ahler manifold $(M,\omega,J;\Sigma)$ we mean a
symplectic manifold $(M^{2n},\omega)$ together with an integrable
$\omega$-compatible complex structure $J$ and a complex hypersurface
$\Sigma$ such that $[\Sigma] \in H_{2n-2}(M)$ is Poincar\'e dual to
$k[\omega] \in H^2(M)$ for some $k \in \mathbb N$. There is an
essentially canonical plurisubharmonic function $\varphi: M
\smallsetminus \Sigma \to \mathbb R$ associated to this data. 

In the following we will concentrate on the case that its critical set
$\mathrm{Crit}\,\varphi$ is a connected submanifold of dimension
$n$. In this case, $(M \smallsetminus \mathrm{Crit}\,\varphi, \omega)$
is symplectomorphic to a standard symplectic disc bundle $E \to
\Sigma$ modeled on the normal bundle of $\pi: N_\Sigma \to \Sigma$ of
$\Sigma$ in $M$. More precisely, there exist a function $r: N_\Sigma
\to \mathbb R_{\geq 0}$ and a 1-form $\alpha$ on $N_\Sigma$ such that
$\omega_{\mathrm{can}} = \pi^*(\omega\vert_\Sigma) + d(r^2 \alpha)$ is
symplectic
. Denoting by $E_\Sigma$ the symplectic disc-subbundle given by $r^2 <
1$, there exists a canonical symplectomorphism $F: (E_\Sigma,
\frac{1}{k} \omega_{\mathrm{can}}) \to (M \smallsetminus
\mathrm{Crit}\,\varphi, \omega)$. We denote by $P_{r_0} = \{x \in M
\smallsetminus \mathrm{Crit}\,\varphi ~|~r(F^{-1}(v)) = r_0\}$ its
circle subbundle of radius $r_0 \in (0,1)$.

The unstable manifolds $W^u_p(X_{\varphi})$ of the gradient vector
field of $\varphi$ are Lagrangian and intersect $P_{r_0}$ transversely
in an $(n-1)$-sphere $S = W^u_p(X_\varphi) \cap P_{r_0}$ which
projects to a Lagrangian sphere $\Lambda$ in $\Sigma$ (the
\emph{trace} of the polarization). Denoting by $\pi_{r_0}: P_{r_0} \to
\Sigma$ the restriction of the canonical projection, we consider the
Lagrangian circle bundle $L = \pi_{r_0}^{-1}(\Lambda)$ over $\Lambda$
at radius $r_0$. By construction, $L$ contains the sphere $S$, and
there is a Lagrangian surgery disc $D$ for $S$ which is given by the
part of $W^u_p(X_\varphi)$ below $S$.

\subsubsection{Example: $(\mathbb CP^n, Q)$}
\label{sec:example:-mathbb-cpn}

An example for this situation is $\mathbb CP^n$ with its standard
K\"ahler structure and where $\Sigma = \{z_0^2 + \dots + z_n^2 = 0\}$
is a quadric. In this case, we have $\mathrm{Crit}\,\varphi = \mathbb
RP^n$ and $\mathbb CP^n \smallsetminus \Sigma$ is symplectomorphic to
the unit cotangent bundle $D^*\mathbb RP^n$ of $\mathbb RP^n$ with
respect to the standard round metric [\textbf{REALLY}?].  

Set $r_0 = 1/\sqrt{n+1}$, which is the unique radius such that the
Lagrangian circle bundle $L = \pi_{r_0}^{-1}(\Lambda)$ is monotone in
$\mathbb CP^n$. Consider now the disc cotangent fibre $D =
D^*_p\mathbb RP^n$; Letting $\hat p$ be the antipodal point


